Maximum Flows in Parametric Graph Templates

Execution graphs of parallel loop programs exhibit a nested, repeating structure. We show how such graphs that are the result of nested repetition can be represented by succinct parametric structures. This parametric graph template representation allows us to reason about the execution graph of a parallel program at a cost that only depends on the program size. We develop structurally-parametric polynomial-time algorithm variants of maximum flows. When the graph models a parallel loop program, the maximum flow provides a bound on the data movement during an execution of the program. By reasoning about the structure of the repeating subgraphs, we avoid explicit construction of the instantiation (e.g., the execution graph), potentially saving an exponential amount of memory and computation. Hence, our approach enables graph-based dataflow analysis in previously intractable settings.

==> sec-fullyparametric.tex <==
\section{Fully Parametric Template Algorithms}

So far, we have focussed on the viewpoint that the parameters are given and fixed, providing polynomial time algorithms, given a set of parameters. However, we can also attempt to characterize the solution-space as a function of the parameters. %A \emph{fully parameteric template algorithm} for problem $L$ is given a template graph $G$ and a set of templates $\mathcal{T}$ and construct a data structure that allows us to answer for a given set of parameters $\mathcal{P}$ the answer to $L$ on $\mathcal{G}=(G, \mathcal{T}, \mathcal{P})$ in $O(1)$ time (or $O(\log n)$ time).

Because edge-reweighting, partial instantiation, and instance merging transform the parameters in an analytical way and their control flow is independent on the parameters, we have already shown how to effectively reduce the fully parametric case to the edge-weight parametric case for maximum flows and minimum cuts. For tree subgraph isomorphism, note that we have already characterized the parameter space, because we have in effect solved the problem for all relevant parameters.

%Next, we discuss which types of templates lead to tractable edge-weight parametric problems for maximum $s$-$t$ flows and minimum cuts.

\subsection{Characterizing the Parameter Space: Tree Subgraph Isomorphism}

Since we considered all $O(k^k)$ relevant ways in which the pattern could reuse every template and counted how many times each occurrence would use a template, we effectively have decided the problem for all parameters. Given a certain set of parameters, we search if there is a solution that matches in a $k$-dimension search tree. This means we can answer the tree subgraph isomorphism question in $O(|\mathcal{T}| k^2 \log k \log n)$ time for each set of parameters after the first one

\subsection{Characterizing the Parameter Space: Mincuts}

We characterize all cuts that can become minimum for certain functions of the parameters.
%
The cuts that arise from the case where no template cross the cut do not change with the parameters, and are the same for all parameters. There can be at most $O(n^2)$ such minimum cuts per template~\cite{DBLP:journals/jacm/KargerS96} and hence $O(n^3)$ such cuts overall. For the other cuts, we need to consider the shape of the edge reweighted graphs that arise.

When all parameters are restricted to have the same value $P$, then the edge reweighted problems that arise in the minimum cut computation are all of the following form: An weight $w(e)$ edge $e$ whose deeper endpoint is at depth $i$ in the template tree gets reweighted to $w'(e)=w(e) P^i$. These problems can be solved using Karger's parametric minimum cut approach~\cite{DBLP:conf/stoc/Karger16} in $O(n^3 m)$ time each, and they produce at most $O(n^3)$ cuts that could become minimum. Since we invoke this algorithm once for each template in the case where some template crosses the cut, the runtime is $O(n^4 m)$.

Another tractable case is when the template tree has height $h=1$ and there are a bounded number of template $|\mathcal{T}|$. Then, the weight $w(e)$ edge that goes into template $T_i$ is reweighted to $w'(e)= w(e) P_i$. This can be seens as a linear combination of $|\mathcal{T}|$ terms (all but one have coefficient $0$. Hence, the runtime using Karger's approach~\cite{DBLP:conf/stoc/Karger16} is $O(mn^{1+|\mathcal{T}|})$ and there are $O(n^{1+|\mathcal{T}|})$ cuts that can become minimum.

\subsection{Characterizing the Parameter Space: Maximum Flow}



==> sec-proofs.tex <==
\section{Correctness Proof with Sibling Edges}\label{sec:sibling-proofs}

\begin{proof}[of \Cref{lem:stcut-structure-sibling}]

The proof is by induction on the number of templates in the parametric graph. If the parametric graph has only a single template, then (since $s$ and $t$ must be in this template) the claim is trivial because the root is repeated only once, by assumption.

Otherwise, let $C=(V_s, V_t)$ be a minimum all-$s$-$t$ cut of the parametric graph $G$ (i.e., $V_s$ contains the vertices assigned to $s$ and $V_t$ those assigned to $t$).
%
Consider an arbitrary template $T_i$ that is a \emph{child of the root template}. Let $B_s$ and $B_t$ contain the boundary vertices of $T_i$ that are in $V_s$ and $V_t$, respectively.

If either $B_s$ or $B_t$ are empty, then it follows immediately that all instances of the vertices that are in $T_i$ are in the same part of $C$ (namely on the side of $s$ if $B_t$ is empty and vice versa).

Otherwise, merging all vertices in $B_s$ into a vertex $s'$ and merging all vertices in $B_t$ into a vertex $t'$ does not change the value of the minimum $s$-$t$ cut. Moreover, if the merged parametric graph has a minimum all-$s$-$t$ cut that puts every instance of every vertex on the same side of the cut, then so does the original parametric graph (because $B_s$ and $B_t$ contain only vertices that belong to the root template and we can "undo" the merging). We thus further assume w.l.o.g. that $B_s$ and $B_t$ contain a single vertex named $s'$ and $t'$, respectively.

Every minimum $s$-$t$ cut must separate $s'$ from $t'$ in the subgraph given by the instances of $T_i$ and the vertices $s'$ and $t'$. We use our induction hypothesis to show that there is a minimum all-$s'$-$t'$ cut in this subgraph that puts all instances of a vertex on the same side of the cut. %The cheapest way to do so is to cut every instance along a minimum $s'-t'$ cut in the subgraph induced by the instance of $T_i$ and the boundary vertices (without any edges between boundary vertices).

We construct the parametric graph $G''$ such that a maximum $s$-$t$ flow in $G''$ can be extended to a flow for all edges that intersect $G_i$ or its siblings. $G''$ has the following template graph: take the subgraph of $G$ induced by $T_i$ together with its boundary vertices, then delete any edges going $s'$ to $t'$. The boundary vertices $s'$ and $t'$ and all vertices that belong to $T_i$ are put into the root template of $G''$ (which has parameter $1$). Moreover, $G''$ has the templates and parameters of the descendants of $T_i$ in $G$. The parametric graph $G''$ contains at least one template less than $G$. Hence, by induction, there is a minimum $s'$-$t'$ cut $C''$ of $G''$ that puts all instances of the same vertex into the same partition. 

Let $f''$ bet the dual maximum $s'$-$t'$ flow corresponding to $C''$ in $G''$. Now, we construct a flow $f$ for the edges that intersect the instance $G_i$ or its siblings and show it is maximum. Along each instance of edge $e$ in $T_i$ we send $f''(e)$ flow. The capacity constraint on the flow is trivially satisfied. The conservation constraint on the flow is satisfied because the sibling functions are bijective: In the instantiated graph, the total flow going in and out of an instance of $v$ is the same as for vertex $v$ for $f''$ in $G''$. The value of the flow $f$ is $P_i \cdot v(f)$.

Now, consider the cut $C'$ were we put every instance of a vertex $v$ in $T_i$ on the same side as $v$ is in $C'$. The value of this cut is $P_i \cdot  v(f)$. By strong duality, this shows that $C$ is a minimum $s'$-$t'$ cut in the graph induced by $G_i$, its siblings, and its boundary nodes. By construction, this cut puts every instance of every vertex on the same side of the cut.

% (By contradiction: Every instance must be cut somewhere. If it is not cut along such a minimum  $P_{s}$-$P_{t}$ cut, we can make the cut cheaper by using a minimum $P_{s}$-$P_{t}$ cut.)

We conclude that all children of the root template can be cut such that every instance of the same vertex is in the same part of the cut. Because the root has a single instance, the statement follows for the root as well.

\end{proof}


\iffalse

\subsection{Maximum Flows}\label{sec:apx:maxflow}



\begin{proof}[Proof of \Cref{lem:stcut-structure}]
The proof is by induction on the number of templates in the parametric graph template. If the parametric graph template has only a single template, then (since $s$ and $t$ must be in this template) the claim is trivial because the root is repeated only once, by assumption.

Otherwise, let $C=(V_s, V_t)$ be a minimum all-$s$-$t$ cut of the parametric graph template $\mathcal{G}$ (i.e., $V_s$ contains the vertices assigned to $s$ and $V_t$ those assigned to $t$).
%
Consider an arbitrary template $T_i$ that is a \emph{child of the root template} and its graph template $G_i$.
%
The sets $B_s$ and $B_t$ contain the boundary vertices of $T_i$ that are in $V_s$ and $V_t$, respectively. 

If either of the sets $B_s$ or $B_t$ is empty, then it follows immediately that all instances of the vertices that are in $T_i$ are in the same part of the cut $C$ (i.e., on the side of $s$ if the set $B_t$ is empty and vice versa). 

Otherwise, merging all vertices in $B_s$ into a vertex $s'$ and merging all vertices in $B_t$ into a vertex $t'$ does not change the value of the minimum $s$-$t$ cut in $\mathcal{G}$. Moreover, if the merged parametric graph template has a minimum $s$-$t$ cut that puts every instance of every vertex on the same side of the cut, then so does the original parametric graph template (because $B_s$ and $B_t$ contain only vertices that belong to the root template and we can ``undo'' the merging). We thus further assume w.l.o.g. that $B_s$ and $B_t$ contain a single vertex named $s'$ and $t'$, respectively. Note that since these vertices belong to the root template, the vertices $s'$ and $t'$ coincide with their only instances.

Every minimum $s$-$t$ cut must separate $s'$ from $t'$ in the subgraph $H$ given by the instances of $T_i$ and the vertices $s'$ and $t'$ (but without a potential edge from $s'$ and $t'$). We use our induction hypothesis to show that there is a minimum $s'$-$t'$ cut in this subgraph that puts all instances of a vertex on the same side of the cut. 

We construct a parametric graph template $\mathcal{G}''$ such that a maximum $s'$-$t'$ flow in $\mathcal{G}''$ can be extended to a flow for the graph $H$. The parametric graph template $\mathcal{G}''$ has the following template graph: take the subgraph of $G$ induced by $T_i$ together with its boundary vertices, then delete any edges going between $s'$ and $t'$. The boundary vertices $s'$ and $t'$ and all vertices that belong to $T_i$ are put into the root template of $\mathcal{G}''$ (which has parameter $1$). Moreover, $\mathcal{G}''$ has the templates and parameters of the descendants of $T_i$ in $G$. The parametric graph template $\mathcal{G}''$ contains at least one template less than $G$. Hence, by induction, there is a minimum $s'$-$t'$ cut $C''$ of $\mathcal{G}''$ that puts all instances of the same vertex into the same partition. 

Let $f''$ be the dual maximum $s'$-$t'$ flow corresponding to $C''$ in $\mathcal{G}''$ of value $\mu$. Now, we construct a $s'$-$t'$ flow $f$ in $H$ and show it is maximum. Along each instance of each edge $e$ that intersects $T_i$ we send $f''(e)$ flow. The capacity constraint on the flow is trivially satisfied. The conservation constraint on the flow is satisfied because in the instantiated graph, the total flow going in and out of an instance of $v$ is the same as for vertex $v$ for $f''$ in $\mathcal{G}''$. The value of the flow $f$ is $P_i \cdot \mu$.

Now, consider the cut $C'$ where we put every instance of a vertex $v$ in $T_i$ on the same side as $v$ is in $C''$. The value of this cut is $P_i \cdot \mu$. By strong duality, this shows that $C'$ is a minimum $s'$-$t'$ cut in the graph $H$. By construction, this cut puts every instance of every vertex on the same side of the cut.

We conclude that all children of the root template can be cut such that every instance of the same vertex is in the same part of the cut. Because the root has a single instance, the statement follows for the root as well.
\end{proof}


\begin{proof}[Proof of \Cref{lem:stcut-reweighting}]
%
Any cut in the reweighted graph $G'$ corresponds to a cut of the same value in the parametric graph template $\mathcal{G}=(G,\mathcal{T}, \mathcal{P})$: Put every instance of a vertex into the partition that it has in the cut of $G'$. Since every edge $e$ is cut exactly $\prod_{i\in I(e)} P_i$ times, this shows that the value of the minimum $s$-$t$ cut of the graph $G'$ is at least the value of the minimum all-$s$-$t$ cut of the parametric graph template $(G,\mathcal{T}, \mathcal{P})$.

It remains to show that the minimum $s$-$t$ cut of the reweighted graph $G'$ is at most the value of the minimum $s$-$t$ cut of the parametric graph template $\mathcal{G}$.
%
By \Cref{lem:stcut-structure}, there is a minimum $s$-$t$ cut $C$ of $\mathcal{G}$ that puts every instance of every vertex on the same side of the cut. Now, we construct a cut $C'$ of $G'$ from this cut $C$ by putting every vertex $v$ in $G'$ on the same side of the cut as all the instances of $v$ are in $C$. 
The cut $C'$ has the same value $\mu$ because every instance of an edge $e$ in $\mathcal{G}$ is crossing $\prod_{i\in I(e)} P_i$ times, which is the amount by which we scaled the weight of edge $e$ in $G'$. 
\end{proof}

\subsection{Minimum Cut}\label{sec:apx:mincut}

\subsubsection{No Template Crosses the Minimum Cut}\label{sec:apx:mincut:nocross}

\begin{proof}[Proof of \Cref{lem:mincut-structure-nocross}]
	The proof is by induction on the number of parameters. Consider a minimum cut $C$ of $\mathcal{G}$ where no template crosses the cut. 
	Consider a vertex $v$ that belongs to an instance $I$, where $v$ is on a different side of the cut $C$ as the boundary vertices of the instance $I$ (if no such vertex exists, all vertices are on the same side of the cut as the boundary vertices of the instances that contain them and we are done). There are two cases:
	
	\miniheading{Case 1} \emph{The instance $I$ has at least one child $I'$.} By assumption, this child $I'$ has its boundary vertices on the same side of the cut. Hence, all vertices in this child instance $I'$ must be on the same side of the cut as the boundary vertices of $I'$, since otherwise one side of the minimum cut would induce at least two connected components (which contradicts its minimality -- If one side of the cut induces at least two connected components, switching one such connected component to the other side reduces the cut value). Therefore, we can merge the child template (which instantiated $I'$) with its boundary vertices and obtain a parametric graph template with fewer parameters and the same minimum cut value. By induction, this graph has a cut with the desired properties. This cut gives us a cut in the original graph with the desired properties (by replacing each vertex with the set of vertices that were merged into it).
	
	\miniheading{Case 2} \emph{The instance $I$ has no children.} In this case, there cannot be any vertices on the same side of $v$ that are not in $I$. If there would be any such vertices, the cut partitions would induce more than two connected components, again contradicting optimality.
	
\end{proof}

\subsubsection{A Template Crosses the Minimum Cut}\label{sec:apx:mincut:cross}

\begin{proof}[Proof of \Cref{lem:mincut-structure-cross} ]
Let $C$ be a minimum cut where some template crosses the cut $C$. Let $T'$ be a topmost template that crosses the cut $C$.  Let $I'$ be an instance of $T'$ with boundary vertices on both sides of the cut. The parent of $I'$ is either the root, or it has boundary vertices on the same side of the cut $C$ (otherwise $T'$ is not topmost). Let $I''$ be the instance found this way and $T''$ be its template. We continue to prove that the template $T''$ is the sought-after template $T$, by exhibiting a cut of the desired form (using \Cref{lem:stcut-structure}).

Let $A$ be the set of vertices on the side of the cut of the boundary vertices of $I''$ and $B$ be the set of vertices on the other side of the cut.
	Observe that the set $B$ is fully contained in the instance $I''$. This follows because $A$ and $B$ must each be a connected subgraph of the instantiation (and there is no way to enter the instance $I''$ without going through the boundary vertices).

Consider the parametric subgraph $\mathcal{G}[T']$ induced by the template $T'$ and its boundary vertices.
%
The sets $A$ and $B$ translate into sets of vertices $A'$ and $B'$ in the template graph $G'$ of the parametric subgraph $\mathcal{G}[T']$ (take for every vertex in the set the vertex that instantiated it). Any cut of $\mathcal{G}[T']$ that has one side of the cut containing $A'$ and the other side of the cut containing $B'$ can be turned into a cut of $\mathcal{G}$ of the same value.
 
In $\mathcal{G}[T']$, merge all the vertices in $A'$ into a single vertex $a$ and merge all the vertices in $B'$ into a single vertex $b$. Consider a minimum $a$-$b$ cut $C_{ab}$ of the merged parametric subgraph with the properties guaranteed by \Cref{lem:stcut-structure}. That is, all instances of the same vertex are on the same side of the cut $C_{ab}$. Undoing the merging gives the desired cut $C'$. This cut has the same value as $C_{ab}$ in $\mathcal{G}[T']$ and hence also $\mathcal{G}$ (Thus the cut $C_{ab}$ has value at least that of $C$). Additionally, since the cut $C$ corresponds to an $a$-$b$ cut in the merged graph, the minimum $a$-$b$ cut $C_{ab}$ has value at most $C$.
\end{proof}
\fi

\iffalse
\subsection{Subgraph Isomorphism}\label{sec:apx:isomorph}

In this section, we prove the correctness and runtime of the subgraph isomorphism algorithm from \Cref{sec:tree-si}.  We begin by showing a property about paths in template-acyclic graphs. We will use the following \Cref{cor:acyc-paths} to show that the algorithm finds all semi-colorful occurrences.

\begin{lemma}
	[Template-Acyclic Paths]\label{cor:acyc-paths}
	In an instantiation of a template-acyclic parametric graph template,
	consider a path $P_{uv}$ from vertex $u$ to vertex $v$
	and a path $P_{wz}$ from vertex $w$ to vertex $z$ where $T(v)=T(z)$. If $~T(v)=T(u)$, or $T(v)$ is an ancestor of $~T(u)$, then if $u$ and $w$ belong to the same instance of the same template, then $v$ and $z$ do as well.
\end{lemma}
\begin{proof}
The proof is by strong induction on the sum of the length of the two paths. If the lengths are $0$, then $u=v$ and $w=z$ and the statement follows immediately. Otherwise, assume as the induction hypothesis that the statement holds for all pairs of paths whose sum of the path lengths are shorter that the sum of the length of $P_{uv}$ and $P_{wz}$.

In a template-acyclic graph, it is impossible (by definition) that there is a path from an instance of a template to another instance of the same template. This proves the case where $T(u)=T(v)$. For the case where $T(v)$ is an ancestor of $T(u)$, recall that paths in an instantiation of a parametric graph template correspond to walks in the template tree. Now, consider the first edge $(x, y)$ in the path $P_{uv}$ where $y$ belongs to an instance of $T(v)$ and the first edge $(x', y')$ in the path $P_{wz}$ where $y'$ belongs to an instance of $T(v)$. By construction, $T(x)=T(x')$ where this template is a child of $T(v)$. Therefore, by induction, $x$ and $x'$ are in the same instance of the same template. Now, since edges can only cross one template instance boundary at a time, $y$ and $y'$ must also be in the same instance of the same template. Apply the induction hypothesis for the path $P_{yv}$ from $y$ to $v$ and the path $P_{y'z}$ from $y'$ to $z$ to conclude the proof.
\end{proof}

\begin{corollary}[Converging Paths]\label{cor:conv-paths}
In an instantiation of a template-acyclic parametric graph template,
	consider an instance $u'$ of vertex $u$ and two instances $v'$ and $v''$ of the same vertex $v$ where either $T(u)=T(v)$ or $T(v)$ is an ancestor of $~T(u)$. If there is a path from $u'$ to $v'$ and a path from $u'$ to $v''$, then $v'=v''$.
\end{corollary}
\begin{proof}
Apply the template-acyclic paths \Cref{cor:acyc-paths} for the path $P_{u'v'}$ and the path $P_{u'v''}$
\end{proof}


\begin{lemma}
	[Completeness]
	If there is a semi-colorful occurrence of the tree $A$ rooted at $x$ using the colors in the set $c$ on its spine, then the set of colors $c$ is in the list $C(A, x)$.
\end{lemma}
\begin{proof}
The proof is by structural induction along the recursive structure of the algorithm.
The base case of the algorithm is clearly correct.
Consider a semi-colorful occurrence of $A$ rooted at $x$ using the colors in the set $c$. Split the tree $A$ into $A'$ and $A''$ as in the algorithm. This yields a semi-colorful occurrence of tree $A'$ rooted at $x$ using a set of colors $c'$ on its spine and a semi-colorful occurrence of $A''$ rooted at a vertex $y$ using a set of colors $c''$ on its spine, where there is an edge $(x, y)$. The induction hypothesis is that the algorithm finds that $c'$ is in $C(A', x)$ and that $c''$ is in $C(A'', y)$. 

\begin{description}
	\item [Case 1. $T(x)$ is a parent of $T(y)$. ] 
	
We need to show that $(c' \cup c'') \setminus c_{\text{low}}$ is the set of colors on the spine of the occurrence of $A$ and that $(c'\setminus c_{\text{low}})$ and  $(c''\setminus c_{\text{low}})$ are disjoint.

In this case, the spine of the occurrence of $A$ contains the spine of the occurrence of $A'$ and the spine of the occurrence of $A''$, without the vertices that belong to $T(y)$. By the induction hypothesis, the sets $c'$ and $c''$ contain colors of the vertices in the spines of the occurrence of $A'$ and $A''$, respectively. Moreover, by definition the color set $c_{\text{low}}$ contains the colors that occur in the template $T(y)$ and no colors that occur in the spine of the occurrence of $A$. Hence, $(c' \cup c'')\setminus c_{\text{low}}$ is indeed the set of colors that occur on the spine of the occurrence of $A$.

To prove that $(c'\setminus c_{\text{low}})$ and  $(c''\setminus c_{\text{low}})$ are disjoint, assume otherwise (for contradiction). Since the occurrence of $A$ is semi-colorful, there must be a vertex $v'$ in the occurrence of $A'$ and a vertex $v''$ in the occurrence of $A''$ that are instances of the same vertex $v$. Since $c_{\text{low}}$ contains the colors in $T(y)$ (and using the induction hypothesis), $(c'\setminus c_{\text{low}})$ and  $(c''\setminus c_{\text{low}})$ must intersect in a color that is in $T(x)$ or an ancestor of $T(x)$. Moreover, there is a path from $x$ to $v'$ (along the occurrence of $A'$) and a path from $x$ to $v''$ (using the edge $(x, y)$ and then along the occurrence of $A''$). Hence, by Converging Paths (\Cref{cor:conv-paths}), $v'=v''$, which contradicts that $A$ is a tree. 
	\item [Case 2. $T(x)=T(y)$ or $T(x)$ is a child of $T(y)$.]
	We need to show that $c' \cup c''$ is the set of colors in the spine of the occurrence of $A$ and that $c'$ and $c''$ are disjoint.

Because $T(x)=T(y)$ or $T(x)$ is a child of $T(y)$, the spine of the occurrence of $A$ contains the spine of the occurrence of $A'$ and the spine of the occurrence of $A''$. Therefore, the set $c' \cup c''$ is indeed the colors of the spine of the occurrence of $A$.

To show that $c'$ and $c''$ are disjoint, assume otherwise (for contradiction). Then, because the occurrence of $A$ is semi-colorful, there is a vertex $v'$ in the spine of the occurrence of $A'$ and a vertex $v''$ in the spine of the occurrence of $A''$ that are both instances of the same vertex $v$. Because $T(x)=T(y)$ or $T(x)$ is a child of $T(y)$, we conclude that $v'$ and $v''$ must either belong to $T(x)$ or an ancestor of $T(x)$. Moreover, there is a path from $x$ to $v'$ and $x$ to $v''$ (along the occurrence of the tree $A'$ and the edge $(x, y)$ followed by a path in the occurrence of $A''$, respectively). Hence, by Converging Paths (\Cref{cor:conv-paths}), $v'$ and $v''$ must be the same vertex, which again contradicts that $A$ is a tree.
\end{description}
\end{proof}


\begin{lemma}[Safety]
	If the list $C(A, x)$ contains the color set $c$, then there is an occurrence of the tree $A$ rooted at $x$ using exactly the colors from the set $c$ on its spine.
\end{lemma}
\begin{proof}[Proof]

The idea is again to proceed by induction. We get two subtrees $A'$ and $A''$ as before where $A'$ is rooted at $x$ and $A''$ at some child of $x$. The induction hypothesis guarantees us that there are occurrences of $A'$ and $A''$ using colors $c'$ and $c''$ on their spines, respectively. We need to prove that there is an occurrence of $A$ using the colors $c$ on its spine as constructed in the algorithm. This involves showing that either the vertices in the two subtrees are distinct, or mapping the occurrences onto other vertices so that this is the case.

Vertices in the spine of the occurrence of $A$ cannot be confused (their occurrences must be distinct) as their colors are distinct.

Outside of the spine of the occurrence of $A$, we can always combine instantiations of $A'$ and $A''$ by choosing different instantiations. Specifically, if there is a potential clash between instances of a vertex $v$ in the occurrences of $A'$ and $A''$, consider the least common ancestor $T'$ of $T(v)$ and $T(x)$. Let $T''$ be the child of $T'$ that contains $v$. There is such a template because $v$ is not in the spine of $A$ and $T(v)$ is the descendant of some template in the spine. 
%
Choose two different instances for the part of $A'$ that is in $T''$ and the part of $A''$ that is in $T''$. This works because $T''$ is not in the spine of $A$, and since there are always enough instances (because we count the number of times a color is reused). 
\end{proof}

\fi 
